Hierarchical quantum classifiers

Quantum circuits with hierarchical structure have been used to perform binary classification of classical data encoded in a quantum state. We demonstrate that more expressive circuits in the same family achieve better accuracy and can be used to classify highly entangled quantum states, for which there is no known efficient classical method. We compare performance for several different parameterizations on two classical machine learning datasets, Iris and MNIST, and on a synthetic dataset of quantum states. Finally, we demonstrate that performance is robust to noise and deploy an Iris dataset classifier on the ibmqx4 quantum computer.

==> figure_1.tex <==
\begin{figure}%[!htb]
    \centering
    \begin{subfigure}[b]{0.495\textwidth}
       \includegraphics[width=\textwidth]{TTN}
       \caption{TTN classifier}
       \label{fig:TTN}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\textwidth}
       \includegraphics[width=\textwidth]{MERA}
       \caption{MERA classifier}
       \label{fig:MERA}
    \end{subfigure}
    \caption{\textit{TTN and MERA classifiers for 8 qubits.} The quantum circuit is illustrated by the regions outlined in solid lines comprising inputs $\psi$, unitary blocks $\{U_i\}_{i=1}^7$ and $\{D_i\}_{i=1}^4$, and a measurement operator $M$. The dashed lines represent its conjugate transpose. The solid and dashed regions together describe a tensor network operating on input $\psi_{1-8}$ and evaluating to the expectation value of observable $M$.}
    \label{fig:networks}
\end{figure}

==> table_accs.tex <==



\begin{table}[!htb]
\centering
\begin{tabular}{lllllll}
\textbf{Classifier} & \textbf{Unitaries} & \textbf{Rotations} & \textbf{Is} $\mathbf{>4}$&\textbf{Is even}& \textbf{0 or 1} & \textbf{2 or 7} \\ \hline
TTN & Simple & Real &$65.59\pm0.57$&$72.17\pm0.89$&$92.12\pm2.17$&$68.07\pm2.42$\\
TTN & General & Real &$74.89\pm0.95$&$83.13\pm1.08$&$99.79\pm0.02$&$97.64\pm1.60$\\
MERA & General & Real &$75.20\pm1.51$&$82.83\pm1.19$&$99.84\pm0.06$&$98.02\pm1.40$\\
Hybrid & General & Real &$76.30\pm1.04$&$83.53\pm0.21$&$\mathbf{99.87}\pm0.02$&$98.07\pm1.46$\\
TTN & Simple & Complex  &$70.90\pm0.73$&$80.12\pm0.64$&$99.37\pm0.12$&$94.09\pm3.37$\\
TTN & General & Complex  &$77.56\pm0.45$&$83.53\pm0.69$&$99.77\pm0.02$&$97.63\pm1.48$\\
MERA & General & Complex    &$\mathbf{79.10}\pm0.90$&$\mathbf{84.85}\pm0.20$&$99.74\pm0.02$&$\mathbf{98.86}\pm0.07$\\
Hybrid & General & Complex &$78.36\pm0.45$&$84.38\pm0.28$&$99.78\pm0.02$&$98.46\pm0.19$\\
Logistic & N/A & N/A &$70.70\pm0.01$&$81.72\pm0.01$&$99.53\pm0.01$&$96.17\pm0.01$\\
\end{tabular}
\caption{\textit{Binary classification accuracy on the MNIST dataset.} Mean test accuracy and one standard deviation are reported for TTN, MERA and hybrid classifiers with five different random initial parameter settings using two different types of unitary parametrization. Hybrid classifiers consist of pre-training a TTN classifier and that transforming it into a MERA classifier by training additional unitaries.}
\label{tab:MNIST-acc}
\end{table}



==> table_complexity.tex <==


\begin{table}[!htb]
\centering
\begin{tabular}{llll}
\textbf{Dimension} & \textbf{Classifier} &\textbf{Qubit encoding} & \textbf{Amplitude encoding}\\ \hline
1D & TTN &  $O(N\chi^5)$ &  $O(N\chi^{N+5})$ \\
& MERA &  $O(N^{6\log_2{\chi}} \chi^4)$ &  $O(N^{6\log_2{\chi}} \chi^{N+4})$ \\
\midrule     
2D & TTN & $O(N^2\chi^5)$  & $O(N^2\chi^{2N+5})$  \\
& MERA & $O(\chi^{11N-16})$  & $O(\chi^{13N-16})$  \\
\end{tabular}
\caption{\textit{Computational complexity of hierarchical quantum classifiers under different data encoding.} The complexities indicate the number of multiplications of scalar numbers required to obtain the measurement outcomes. We use $N \chi$-dimensional qudits in one dimension and $N \times N$ $\chi$-dimensional qudits in two dimensions.}
\label{tab:complexity}
\end{table}



==> table_iris.tex <==

\begin{table}[!htb]
\centering
\begin{tabular}{llllll}
\textbf{Classifier} & \textbf{Unitaries} & \textbf{Rotations} & \textbf{1 or 2} & \textbf{2 or 3} & \textbf{1 or 3} \\ 
\hline
TTN & Simple & Real & $100.00\pm 0.00$ & $96.77\pm 0.00$ & $100.00\pm 0.00$  \\                                          
\end{tabular}
\caption{\textit{Binary classification accuracy on the Iris dataset.} Mean test accuracy and one standard deviation are reported for TTN classifiers with five different random parameter initializations. The Iris dataset consists of three classes. From these we constructed three binary classification tasks.}
\label{iris-pid}
\end{table}


==> table_synthetic.tex <==
\begin{table}[!htb]
\centering
\begin{tabular}{llllll}
\textbf{Classifier} & \textbf{Unitaries} & \textbf{Rotations} & \textbf{1 or 10} & \textbf{3 or 10}  & \textbf{2 or 5} \\ \hline
TTN & General & Complex & $50.25	\pm	0.58	$&$	49.95\pm	0.72	$&$	50.36	\pm	1.05	$ \\
TTN & Ancilla & Complex & $\mathbf{64.05}	\pm	1.12	$&$	\mathbf{59.33}	\pm	0.22	$&$	\mathbf{58.02}	\pm	0.65$\\
\end{tabular}

\caption{\textit{Binary classification test accuracy on synthetic quantum datasets.} Mean test accuracy and one standard deviation are reported for TTN classifiers with five different random initial parameter settings using two different types of unitary parametrization.}
\label{tab:depth-acc}
\end{table}

